Privileged observations enable rapid and reliable policy discovery directly in the physical world

We study how privileged information about a physical system affects the discovery of high-performing policies when training a reinforcement learning agent directly in the physical world. We let the agent control a cylinder in a tabletop water channel to maximize or minimize drag. The flow is chaotic and difficult to model or simulate accurately and good strategies are not obvious beforehand. Decades-old experimental studies provide recipes for simple, high-performance, periodic open-loop policies that increase drag by 26.6% +/- 0.7% and reduce it by 29.7% +/- 1.3%. With dense observations of the cylinder wake, the agent learns within tens of minutes policies that increase drag by 25.5% +/- 0.9% and reduce it by 32.4% +/- 1.6%. We record action trajectories during online policy execution and replay them open loop as fixed sequences; these replays increase drag by 23.2% +/- 2.2% and reduce it by 32.1% +/- 3.0%. However, when we withhold flow observations during training, the agent still learns to decrease drag by 31.4% +/- 2.1%, but no run learns to increase it (1.8% +/- 4.3% drag increase). Our physical experiments demonstrate an extreme case: privileged observations can be decisive for policy discovery even when the resulting actions can be replayed in open loop.

==> figures/Figure_1.tex <==
\PFFPanel{a}{.31\linewidth}{\includegraphics[width=\linewidth]{images/fluids/intuitive_experiment/game1.jpg}}
\hfill
\PFFPanel{b}{.31\linewidth}{\includegraphics[width=\linewidth]{images/fluids/intuitive_experiment/game2.jpg}}
\hfill
\PFFPanel{c}{.31\linewidth}{\includegraphics[width=\linewidth]{images/fluids/intuitive_experiment/game3.jpg}}


==> figures/Figure_2.tex <==
\includegraphics[trim={75 150 0 150},clip,width=\linewidth]{images/fluids/wake-compress.jpg}


==> figures/Figure_3.tex <==
\begin{minipage}{\linewidth}
    \hfill
    \begin{minipage}{.49\linewidth}
        \centering
        \PFFPanelLetter{a}
        \includegraphics[width=\linewidth,trim={4.8cm 12.5cm 5.2cm 6.5cm},clip]{images/fluids/setup.pdf}
    \end{minipage}
        \hfill
    \begin{minipage}{.49\linewidth}
        \centering
        \PFFPanelLetter{b}
        \includegraphics[trim={40 400 10 0},clip,width=\linewidth]{images/fluids/diagram.pdf}
    \end{minipage}
    \end{minipage}

    \begin{minipage}{\linewidth}
    \centering
    \PFFPanelLetter{c}
    \includegraphics[width=.19\linewidth]{images/fluids/snapshots/1.png}
    \hfill
    \includegraphics[width=.19\linewidth]{images/fluids/snapshots/2.png}
    \hfill
    \includegraphics[width=.19\linewidth]{images/fluids/snapshots/3.png}
    \hfill
    \includegraphics[width=.19\linewidth]{images/fluids/snapshots/4.png}
    \hfill
    \includegraphics[width=.19\linewidth]{images/fluids/snapshots/5.png}
    \end{minipage}


==> figures/Figure_4.tex <==
\begin{tikzpicture}
  \node[anchor=south west,inner sep=0] (img) at (0,0)
    {\includegraphics[width=\linewidth]{images/fluids/flow-cylinder.pdf}};

  \begin{scope}[x={(img.south east)},y={(img.north west)}]
    \node[font=\footnotesize] at (0.5,0.65) {$\mathcal{C}$};
    \node[font=\footnotesize] at (0.5,0.8) {$\partial\mathcal{C}$};

    \draw[->,thick] (0.08,0.95) --
      node[above right,font=\footnotesize] {$\vec{n}_{\infty}$} (0.08,0.78);
    \coordinate (C) at (0.53,0.61);
    \begin{scope}[shift={(C)}]
      \draw[->,thick]
        (60:0.19) arc[start angle=60,end angle=-40,radius=0.19];
    \end{scope}
    \node[font=\footnotesize] at (0.78,0.5) {$\omega(t)$};
    \fill (0.3,0.45) circle (0.8pt);
    \node[font=\footnotesize,anchor=west] at (0.27,0.45) {$\vec x$};
    \node[font=\footnotesize] at (0.15,0.38) {$p(t,\vec x)$};

  \end{scope}
\end{tikzpicture}


==> figures/Figure_5.tex <==
\begin{tikzpicture}
  \node[anchor=south west,inner sep=0] (art) at (0,0)
    {\includegraphics[width=\linewidth]{images/fluids/system.pdf}};
  \begin{scope}[x={(art.south east)},y={(art.north west)}]
    \node[anchor=south west,inner sep=0] at (0,1.02) {\PFFPanelText{a}};
    \node[anchor=south west,inner sep=0] at (.52,1.02) {\PFFPanelText{b}};
  \end{scope}
\end{tikzpicture}


==> figures/Figure_6.tex <==
\includegraphics[width=\linewidth]{images/fluids/learning_curves/legend.pdf}
    \begin{minipage}{0.49\linewidth}
    \PFFPanelLetter{a}
    \includegraphics[width=\linewidth]{images/fluids/learning_curves/max.pdf}

  \end{minipage}
  \hfill
  \begin{minipage}{0.49\linewidth}
    \PFFPanelLetter{b}
    \includegraphics[width=\linewidth]{images/fluids/learning_curves/min.pdf}%

  \end{minipage}


==> figures/Figure_7.tex <==
\includegraphics[width=\linewidth]{images/fluids/online-replay/legend.pdf}
    \begin{minipage}{0.49\linewidth}
    \PFFPanelLetter{a}
    \includegraphics[width=\linewidth]{images/fluids/online-replay/training-curves/max.pdf}

      \PFFPanelLetter{c}

      \includegraphics[width=\linewidth]{images/fluids/online-replay/episode-curves/max.pdf}

  \end{minipage}
  \hfill
  \begin{minipage}{0.49\linewidth}
    \PFFPanelLetter{b}
    \includegraphics[width=\linewidth]{images/fluids/online-replay/training-curves/min.pdf}

      \PFFPanelLetter{d}

      \scalebox{1}[1.03]{\includegraphics[width=\linewidth]{images/fluids/online-replay/episode-curves/min.pdf}}

  \end{minipage}


==> figures/Figure_8.tex <==
\begin{tikzpicture}
  \node[anchor=south west,inner sep=0] (art) at (0,0)
    {\includegraphics[width=\linewidth]{images/fluids/PIV_inv.pdf}};
  \begin{scope}[x={(art.south east)},y={(art.north west)}]
    \node[anchor=south west,inner sep=0] at (0,1.01) {\PFFPanelText{a}};
    \node[anchor=south west,inner sep=0] at (.065,.325) {\PFFPanelText{b}};
    \node[anchor=south west,inner sep=0] at (.51,.325) {\PFFPanelText{c}};
  \end{scope}
\end{tikzpicture}


==> figures/Supplementary_Figure_1.tex <==
\includegraphics[width=\linewidth]{images/fluids/learning_curves/legend.pdf}
    \begin{minipage}{0.49\linewidth}
    \PFFPanelLetter{a}
    \includegraphics[width=\linewidth]{images/fluids/ablations/observation-sets/max.pdf}

  \end{minipage}
  \hfill
  \begin{minipage}{0.49\linewidth}
    \PFFPanelLetter{b}
    \includegraphics[width=\linewidth]{images/fluids/ablations/observation-sets/min.pdf}

  \end{minipage}


==> figures/Supplementary_Figure_2.tex <==
\includegraphics[width=\linewidth]{images/fluids/ablations/model-size/legend.pdf}

    \begin{minipage}{.49\linewidth}
    \PFFPanelLetter{a}
    \includegraphics[width=\linewidth]{images/fluids/ablations/model-size/max_D_R.pdf}

    \end{minipage}
\hfill
    \begin{minipage}{.49\linewidth}
    \PFFPanelLetter{b}
    \includegraphics[width=\linewidth]{images/fluids/ablations/no-flow/max_D_R.pdf}

    \end{minipage}


==> figures/Supplementary_Figure_3.tex <==
\includegraphics[height=0.8cm]{images/fluids/ablations/rl/legend.pdf}

    \begin{minipage}{.49\linewidth}
    \centering
        \PFFPanelLetter{a}
\includegraphics[width=\linewidth]{images/fluids/ablations/rl/rl.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}{.49\linewidth}
    \centering
        \PFFPanelLetter{b}
\includegraphics[width=\linewidth]{images/fluids/ablations/rl/rl_long.pdf}
    \end{minipage}


==> figures/legends.tex <==
% Each legend has a content title and a separate descriptive body.


\PFFDeclareFigureLegend{1}{Visual observations during a paper-ball game.}{%
\textbf{a)} A participant prepares a crumpled paper ball, throws it, and observes where it lands.
\textbf{b)} The participant closes their eyes and walks toward the remembered location.
\textbf{c)} The participant reaches for the ball; a brief visual observation can help correct the remaining error.}

\PFFDeclareFigureLegend{2}{Wake behind the cylinder.}{%
The cylinder is visible at the left, and the wake, illuminated by the laser, extends to the right within the water-channel test section. This image provides a qualitative view of the physical flow used in the experiments.}

\PFFDeclareFigureLegend{3}{Water-channel apparatus and flow observations.}{%
\textbf{a)} Our tabletop \glsentrylong{cwc} (\glsentryshort{cwc}) with close-ups of the main components. Setup photograph by Thomas Bi.
\textbf{b)} Top and front views of the channel. The channel consists of an upper and a lower branch. The test section (\textbf{1}) in the upper branch houses the cylinder (\textbf{2}). \PFFProtocolPropellerCount{} APISQUEEN U5 brushless freshwater propellers (\textbf{3}) drive a left-to-right flow. Guide vanes (\textbf{4}) redirect the flow into the lower branch and then back to the upper branch. A honeycomb structure (\textbf{5}) straightens the flow and suppresses large-scale vortices. Flow restrictions (\textbf{6}) accelerate the stream and stretch remaining small-scale vortices. The imaging setup (\textbf{7}) produces real-time flow field estimates.
\textbf{c)} Five consecutive snapshots of the estimated flow field, ordered from left to right.
Red and blue indicate positive and negative vorticity, respectively, computed from the estimated flow fields. Arrows represent velocity vectors.}

\PFFDeclareFigureLegend{4}{Flow around a rotating cylinder.}{%
The cylinder $\mathcal{C}$ has boundary $\partial\mathcal{C}$ and commanded angular velocity $\omega(t)$. The vector $\vec n_{\infty}$ denotes the incoming-flow direction, and $p(t,\vec x)$ is the fluid pressure at position $\vec x$ and time $t$.}

\PFFDeclareFigureLegend{5}{System overview.}{%
\textbf{a)} Physical system. Setup photograph by Thomas Bi. \textbf{b)} Controller.
The \mbox{\glsentrylong{rl} (\glsentryshort{rl})} agent commands the cylinder rotation rate. It receives the previous command, the drag measurement, motor rotation-rate feedback, and, in the augmented observation set, the dense flow field estimate. We compare training performance under these observation sets.}

\PFFDeclareFigureLegend{6}{Training with and without flow observations.}{%
\textbf{a)} Drag-maximization training with \texttt{DreamerV3}.
\textbf{b)} Drag-minimization training with the same algorithm.
The vertical axes show episode-average filtered-drag change, expressed as a percentage of the no-control mean; positive values indicate increased drag and negative values indicate reduced drag. The horizontal axes show active training time in minutes (min).
Blue solid lines represent supplied flow observations, and red solid lines represent withheld flow observations. Solid lines show means across \PFFProtocolMainRepetitions{} independent training runs, and matching shaded bands show the minimum-to-maximum ranges.
Black dashed lines mark zero drag change without control; black dotted lines mark the task's selected high-performing sinusoidal reference.}

\PFFDeclareFigureLegend{7}{Online policy execution and open-loop replay.}{%
\textbf{a)} Episode-average filtered-drag change during drag-maximization training.
\textbf{b)} The corresponding drag-minimization training record.
\textbf{c)} Within-episode running mean of filtered-drag change for drag maximization after \PFFPaperReplayPanelTrainingMinutes{} minutes of training.
\textbf{d)} The corresponding running mean for drag minimization at the same training checkpoint.
The vertical axes express drag change as a percentage of the no-control mean. The horizontal axes show active training minutes (min) in a) and b), and elapsed episode time in seconds (s) in c) and d). Each running mean starts at the first sample of its episode.
Blue solid lines show online execution. Orange solid lines show the mean of \PFFProtocolReplayRepeats{} physical open-loop replays of the recorded action trajectory; orange shaded bands show their minimum-to-maximum ranges.
Black dashed lines mark zero drag change without control, and black dotted lines mark the selected high-performing sinusoidal reference.}

\PFFDeclareFigureLegend{8}{Camera and laser timing for flow estimation.}{%
\textbf{a)} Timing diagram for camera exposure and laser illumination. The blue line is high while the camera shutter is open and low while it is closed. The red line is high during a laser pulse and low between pulses. The horizontal black arrow is the time axis $t$. The symbols $t_0$ and $t_1$ identify the acquisition times of the first images in two successive pairs; $\Delta t$ is the time separation within each pair. Grey dashed guides mark pulse timing and link the first pair to its images.
\textbf{b)} Tracer-particle image captured at $t_0$.
\textbf{c)} The paired image captured at $t_0+\Delta t$.
Dark spots depict tracer particles. Their displacement between the two images, divided by the elapsed time, provides the flow-velocity estimate used in \glsentrylong{piv} (\glsentryshort{piv}).}

\PFFDeclareFigureLegend{S1}{Training across observation configurations.}{%
\textbf{a)} Drag-maximization results aggregated over observation configurations.
\textbf{b)} The corresponding drag-minimization results.
The vertical axes show episode-average filtered-drag change as a percentage of the no-control mean; the horizontal axes show active training time in minutes (min).
Red marks configurations with flow observations withheld, and blue marks configurations with flow observations supplied. Coloured circles show means across configuration means; pale bands span the first to third quartiles, or the middle half of the configuration means. Vertical whiskers show their minimum-to-maximum ranges; red dashed whiskers denote withheld observations and blue solid whiskers denote supplied observations. Thin black segments connect successive mean values.
The main configurations have \PFFProtocolMainRepetitions{} repetitions and each additional configuration has \PFFProtocolDreamerAdditionalRepetitions{} repetitions; available repetitions are averaged within each configuration before aggregation.
Black dashed horizontal lines mark no control, and black dotted horizontal lines mark the selected high-performing sinusoidal reference.}

\PFFDeclareFigureLegend{S2}{Model size and implementations for withholding flow observations.}{%
\textbf{a)} Drag-maximization training with a \PFFProtocolSmallModelParametersMillions-million-parameter \texttt{DreamerV3} model (teal) and the standard \PFFProtocolStandardModelParametersMillions-million-parameter model (red), both with the flow-observation branch omitted.
\textbf{b)} The standard model with its flow-observation input fixed to zero (dark grey), compared with omission of that branch (red).
The vertical axes show episode-average filtered-drag change as a percentage of the no-control mean; the horizontal axes show active training time in minutes (min). Solid lines show means across repetitions, and matching shaded bands show the minimum-to-maximum ranges. The red reference uses \PFFProtocolMainRepetitions{} repetitions, the smaller model uses \PFFProtocolDreamerModelSizeRepetitions{}, and the zero-input model uses \PFFProtocolDreamerZeroedFlowRepetitions{}.
Black dashed lines mark no control, and black dotted lines mark the selected high-performing sinusoidal reference.}

\PFFDeclareFigureLegend{S3}{Drag-maximization training with alternative learning algorithms.}{%
\textbf{a)} Training over the common \PFFProtocolAlgorithmBudgetMinutes-minute budget with \glsentrylong{ppo} (\glsentryshort{ppo}, green), \glsentrylong{ppor} (\glsentryshort{ppor}, yellow), and \glsentrylong{sac} (\glsentryshort{sac}, magenta). Solid lines show means across \PFFProtocolAlgorithmRepetitions{} independent repetitions, and matching shaded bands show minimum-to-maximum ranges.
\textbf{b)} One extended \glsentryshort{sac} training run over \PFFProtocolExtendedSACHours{} hours, shown as a magenta solid line without a variability band.
The vertical axes show episode-average filtered-drag change as a percentage of the no-control mean; the horizontal axes show active training time in minutes (min). Black dashed lines mark no control, and black dotted lines mark the selected high-performing sinusoidal reference. \Cref{appendix:experimental-accounting} gives the experimental accounting.}


==> figures/manifest.tex <==
% Export identifier, manuscript reference label, standalone artwork width.
\PFFDeclareFigure{1}{fig:intuitive-game}{100mm}
\PFFDeclareFigure{2}{fig:cover}{130mm}
\PFFDeclareFigure{3}{fig:hardware_overview}{180mm}
\PFFDeclareFigure{4}{fig:cylinder-schematic}{50mm}
\PFFDeclareFigure{5}{fig:system}{180mm}
\PFFDeclareFigure{6}{fig:training-curves}{180mm}
\PFFDeclareFigure{7}{fig:results:feedforward:lc}{180mm}
\PFFDeclareFigure{8}{fig:piv-timing}{65mm}
\PFFDeclareSupplementaryFigure{1}{fig:observations-all}{180mm}
\PFFDeclareSupplementaryFigure{2}{fig:ablations:architecture}{180mm}
\PFFDeclareSupplementaryFigure{3}{fig:ablations:rl}{180mm}


==> generated/tables/negative_response.tex <==
% Generated by code/paper/build_paper_numbers.py.
% Do not edit this file by hand.
\ifdefined\PFFPaperNumbersLoaded\else
  \PackageError{paper_numbers}{Load paper_numbers.tex before negative_response.tex}{The generated fragment requires the centralized paper-number registry.}
  \expandafter\endinput
\fi
{Online \texttt{DreamerV3}} & {$4641/4918$ $(94.4\%)$} & {$1049/1092$ $(96.1\%)$} \\
{Mean of five paired replays} & {$360/360$ $(100.0\%)$} & {$161/161$ $(100.0\%)$} \\
{Open-loop grid condition means, incoming flow} & {$92/129$ $(71.3\%)$} & {$3/19$ $(15.8\%)$} \\
{Higher-frequency sinusoidal condition means} & {$11/11$ $(100.0\%)$} & {Not applicable} \\
{Online \texttt{DreamerV3}, flow-observation input zeroed} & {$159/180$ $(88.3\%)$} & {$10/10$ $(100.0\%)$} \\
{One-million-parameter \texttt{DreamerV3}} & {$180/180$ $(100.0\%)$} & {Not applicable} \\
{\PFFProtocolAlgorithmBudgetMinutes-minute learning-algorithm baselines} & {$256/270$ $(94.8\%)$} & {Not applicable} \\
{Open-loop grid condition means, no incoming flow} & {$0/129$ $(0.0\%)$} & {Not applicable} \\

